Risk-Constrained Thompson Sampling for CVaR Bandits

The multi-armed bandit (MAB) problem is a ubiquitous decision-making problem that exemplifies the exploration-exploitation tradeoff. Standard formulations exclude risk in decision making. Risk notably complicates the basic reward-maximising objective, in part because there is no universally agreed definition of it. In this paper, we consider a popular risk measure in quantitative finance known as the Conditional Value at Risk (CVaR). We explore the performance of a Thompson Sampling-based algorithm CVaR-TS under this risk measure. We provide comprehensive comparisons between our regret bounds with state-of-the-art L/UCB-based algorithms in comparable settings and demonstrate their clear improvement in performance. We also include numerical simulations to empirically verify that CVaR-TS outperforms other L/UCB-based algorithms.

==> raw/acknowledgements.tex <==
TBC

==> raw/acknowledgements_personal.tex <==
While these acknowledgements cannot appear in the formal submission to any official forum, I would still like to thank many, many people along the way for their invaluable guidance and support.
\begin{enumerate}
	\item The Holy Spirit. For leading me into UROPS, guiding me every step of the way, and leading me to complete it by His grace.
	\item A/P Vincent Tan and Qiuyu, for their invaluable guidance in supplying the big-picture ideas as well as the careful bookkeeping computations.
	\item My bible study friends for cheering me on and constantly praying for me to walk by grace.
	\item My fellow math friends whom have been through the UROPS process and encouraged me to stay the course and to forge through the failures.
	\item My family, for understanding my moments of pressure and frustration when I spend hours on end without socialising with them.
	\item My life group, for hearing me complain about UROPS every week.
\end{enumerate}

==> raw/proof_of_F_to_0.tex <==
Recall that $c_\alpha^* \to +\infty$ and $c_\alpha^* (1-\alpha) \to 0$. Then $$c_\alpha^*(2-\alpha) =c_\alpha^*(1-\alpha) + c_\alpha^* \to 0 + \infty = +\infty \Rightarrow \frac{1}{c_\alpha^*(2-\alpha)} \to 0.$$
Furthermore, since $$(1-\alpha)c_\alpha(i) = \mu_i \alpha + \sigma_i c_\alpha^*(1-\alpha) $$ implies $$(1-\alpha)\Delta_{\mathrm{r}}(i,\alpha) = \mu_i \alpha + \sigma_i c_\alpha^*(1-\alpha) - c_\alpha(1)(1-\alpha) \to \mu_i-\mu_1,$$ we have
\begin{align*}
\frac{\sigma_i c_\alpha^*}{\Delta_{\mathrm{r}}(i,\alpha)}
&= \frac{\sigma_i c_\alpha^*(1-\alpha)}{(1-\alpha)\Delta_{\mathrm{r}}(i,\alpha)} \to \frac{\sigma_i \cdot 0}{\mu_i-\mu_1} =0.
\end{align*}
Hence, $\xi_\alpha =1 - \frac{\sigma_i c_\alpha^*}{\Delta_{\mathrm{r}}(i,\alpha)} \paren{1 - \frac{1}{c_\alpha^*(2-\alpha)}} \to 1 - 0(1- 0) = 1$.
 Thus,
 \begin{align*}
 \frac{\sigma_i c_\alpha^*}{\sigma_i c_\alpha^* - (1-\xi_\alpha)\Delta_{\mathrm{r}}(i,\alpha)}
 &=  \frac{\sigma_i c_\alpha^*}{\sigma_i c_\alpha^* - \sigma_i c_\alpha^* \paren{1 - \frac{1}{c_\alpha^*(2-\alpha)}}} =  \frac{1}{1 - \paren{1 - \frac{1}{c_\alpha^*(2-\alpha)}}} = c_\alpha^*(2-\alpha) \to +\infty,
 \end{align*}
 and $h(c_\alpha^*(2-\alpha)) \to +\infty$. Finally,$$B_{\alpha,\xi_\alpha}^i = \frac{1}{h \paren{\frac{\sigma_i^2 {(c_\alpha^*)}^2}{{(\sigma_i c_\alpha^* - (1-\xi_\alpha)\Delta_{\mathrm{r}}(i,\alpha))}^2}}} = \frac{1}{h(c_\alpha^*(2-\alpha))} \to 0,$$ as required.



==> raw/proof_of_F_to_0/display.tex <==
\input{Template}

\begin{document}

\section{Bug-fixing}

\input{progress}

\end{document}

==> raw/proof_of_F_to_0/progress.tex <==
Try 
\begin{enumerate}
	\item $\xi_\alpha = 1 - (1-\alpha) {(c_\alpha^*)}^2$,
	\item $\xi_\alpha = 1 - \frac{\sigma_i c_\alpha^*}{\Delta_{\mathsf{risk}}(i,\alpha)} \paren{1 - \frac{1}{c_\alpha^*(2-\alpha)}}$.
\end{enumerate}

Proof of 2

Recall that $c_\alpha^* \to +\infty$ and $c_\alpha^* (1-\alpha) \to 0$. Then $$c_\alpha^*(2-\alpha) =c_\alpha^*(1-\alpha) + c_\alpha^* \to 0 + \infty = +\infty \Rightarrow \frac{1}{c_\alpha^*(2-\alpha)} \to 0.$$
Furthermore, since $(1-\alpha)c_\alpha(i) = \mu_i \alpha + \sigma_i c_\alpha^*(1-\alpha) \Rightarrow (1-\alpha)\Delta_{\mathsf{risk}}(i,\alpha) = \mu_i \alpha + \sigma_i c_\alpha^*(1-\alpha) - c_\alpha(1)(1-\alpha) \to \mu_i-\mu_1$, we have
\begin{align*}
\frac{\sigma_i c_\alpha^*}{\Delta_{\mathsf{risk}}(i)}
&= \frac{\sigma_i c_\alpha^*(1-\alpha)}{\mu_i \alpha + \sigma_i c_\alpha^*(1-\alpha) - c_\alpha(1)(1-\alpha)} \to \frac{\sigma_i \cdot 0}{\mu_i-\mu_1} =0.
\end{align*}
Hence, $\xi_\alpha =1 - \frac{\sigma_i c_\alpha^*}{\Delta_{\mathsf{risk}}(i,\alpha)} \paren{1 - \frac{1}{c_\alpha^*(2-\alpha)}} \to 1 - 0(1- 0) = 1$.
 Thus,
 \begin{align*}
 \frac{\sigma_i c_\alpha^*}{\sigma_i c_\alpha^* - (1-\xi_\alpha)\Delta_{\mathsf{risk}}(i,\alpha)}
 &=  \frac{\sigma_i c_\alpha^*}{\sigma_i c_\alpha^* - \sigma_i c_\alpha^* \paren{1 - \frac{1}{c_\alpha^*(2-\alpha)}}}\\
  &=  \frac{1}{1 - \paren{1 - \frac{1}{c_\alpha^*(2-\alpha)}}}\\
  &= c_\alpha^*(2-\alpha) \to +\infty,
 \end{align*}
 and $h(c_\alpha^*(2-\alpha)) \to +\infty$. Finally,$$B_{\alpha,\xi_\alpha}^i = \frac{1}{h \paren{\frac{\sigma_i^2 {(c_\alpha^*)}^2}{{(\sigma_i c_\alpha^* - (1-\xi_\alpha)\Delta_{\mathsf{risk}}(i,\alpha))}^2}}} = \frac{1}{h(c_\alpha^*(2-\alpha))} \to 0,$$ as required.


